Equilibrium susceptibilities of superparamagnets: longitudinal & transverse, quantum & classical

The equilibrium susceptibility of uniaxial paramagnets is studied in a unified framework which permits to connect traditional results of the theory of quantum paramagnets, $\Sm=1/2, 1, 3/2$, ..., with molecular magnetic clusters, $\Sm\sim5, 10, 20$, all the way up, $\Sm=30, 50, 100$,... to the theory of classical superparamagnets. This is done using standard tools of quantum statistical mechanics and linear response theory (the Kubo correlator formalism). Several features of the temperature dependence of the susceptibility curves (crossovers, peaks, deviations from Curie law) are studied and their scalings with $\Sm$ identified and characterized. Both the longitudinal and transverse susceptibilities are discussed, as well as the response of the ensemble with anisotropy axes oriented at random. For the latter case a simple approximate formula is derived too, and its range of validity assessed, so it could be used in modelization of experiments.

==> paleta.tex <==
%
%
\footnote{
%
We did not consider any interactions between the (super)paramagnetic
entities; our aim was to deepen our knowledge of the superparamagnetic
``ideal gas''.
%
} %END OF FOOTNOTE


Now it is immediate to write down explicit expressions for the
equilibrium susceptibility.
%
Here we will do it for what we called response observables in
Sec.~\ref{avg:response}, and then particularize those general
expressions to ``ladder perturbations'', which include simple
mechanical oscillators and uniaxial paramagnets.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%   SUSCEPTIBILITY:  GENERAL   %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%   SUSCEPTIBILITY:  GENERAL   %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%   SUSCEPTIBILITY:  GENERAL   %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{general $\X$}

The expansion coefficients~(\ref{Z:pert:expl}) of the partition
function can directly be plugged into Eq.~(\ref{X:Z:der}), to
produce explicit formulas for the susceptibility:
%
$\X
=
\beta
\big[
(\Z_{2}/\Z_{0})
-
(\Z_{1}/\Z_{0})^{2}
\big]$.
%
Recall that this form was generic for ``response observables'', when
$\X = \partial_{\bp} \llangle \VQ \rrangle$ with
$\VQ=-\partial_{\bp}\Htot$.
%
Examples included a coordinate, $-x\,F$, a spin component, $-\Sz\Bz$,
etc.


%
%
\footnote{
%
If one considers interactions between the superparamagnetic entities
(dipole-dipole mainly), the whole thing can be scaled up, with
``super'' players, instead of the microscopic spins, leading to
super-ferromagnetism, super-spin-glass, etc.
%
We'll keep it simple, trying to deepen our understanding of the
``ideal gas'' of non-interacting superparamagnets.
%
} %END OF FOOTNOTE


% roman
(cf.~\cite[App.~A]{lopetal2005}).


[Eqs.~(\ref{Xlo}) and~(\ref{Xtr})]


[Eqs.~(\ref{Xran:approx}) and~(\ref{Xran:approx:compact})]


SP: systems described by Huni w large ``S''

$\Hs=-\K\Sz^{2}-\Sz\,\Bz$

longitudinal \& transverse

$\Xlo$ and $\Xtr$

Curie law 

$\Xc=\SSp/3\kT$

$\Xc=\third\beta\SSp$

Ising

$\Xising=\beta S^{2}$

$\Xising=S^{2}/\kT$

T times X

$\kT\Xlo$

spins and powers

$\forall\,S$

$\third\SSp$

$S^{2}$

small spins

$S=1$ and $S=3/2$

scaling 

\kT/\K\,S^{2}

1/S\to0

boltzmania

\e^{-\bEm}

\e^{-\beta\el_{\m}}

\exp(-\beta\K\,\m^{2})

temperaturica

T_{\rm I}\bydefl\tf_{S,S-1}=\K(2S-1)


\Omega\bydefl\beta\tf_{S,S-1}\beta\K(2S-1)

$\llangle \VQ \rrangle
=
\kT
\partial_{\bp}
\Z/\Z$

$\kT\partial_{\bp}\Z=\partial_{(\beta\bp)}\Z\equiv\Z'$



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   INTRODUCTION    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   INTRODUCTION    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   INTRODUCTION    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   INTRODUCTION    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   INTRODUCTION    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   INTRODUCTION    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   INTRODUCTION    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}

\subsection{quantum \& classical (super)paramagnets}

%
%% %
%% \footnote{
%% %
%% By now virtually every quantum system has been proposed as support for
%% quantum information technologies.
%% %
%% Anyway, single-molecule magnets seem more reasonable candidates than
%% quantum black holes \cite{scienceBH}.
%% %
%% } %END OF FOOTNOTE


\subsection{equilibrium susceptibility: from Van Vleck to Transfer matrix}

\subsection{the gap: in this work}


FIGURE LEVELS

%_____________________________
%_____________________________
%_____________________________
\begin{figure}[!t]
%
\centerline{
\includegraphics[width=7.2cm]{el-S2-B0.eps}
\hspace*{-1.ex}
\includegraphics[width=7.2cm]{el-S2-B1.eps}
}
%
\caption{
%
Energy levels $\el_{\m}=-\K\m^{2}-\Bz\m$ of an anisotropic $S=2$ spin.
%
Left: positive anisotropy $\K=1$ at zero field (bistable case).
%
Right: negative $\K=-1$ at the first crossing field $\Bz=|\K|$.
%
}
\label{fig:levels}
\end{figure}
%_____________________________
%_____________________________
%_____________________________



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DERIVATION    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DERIVATION    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DERIVATION    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DERIVATION    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DERIVATION    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DERIVATION    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DERIVATION    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{derivation of the susceptibility}

\subsection{statistical mechanical preliminaries}




average $\VQ$
%_____________________________
%
% AVERAGED QUANTITY
%_____________________________
\begin{equation}
\label{average}
%%%%%%%%%%%%%%%%%%
\llangle \VQ \rrangle
=
\Tr\,
\big(
\dm\,
\VQ)
%%%%%%%%%%%%%%%%%%
\;.
\end{equation}
%_____________________________
%_____________________________



For consistency of the definition (the average of a constant, has to
be the constant itself), $\dm$ is ``normalized'' to have unit trace
%_____________________________
%
% DENSITY MATRIX
%_____________________________
\begin{equation}
\label{density:matrix}
%%%%%%%%%%%%%%%%%%
\dm
=
\e^{-\beta\Htot}
/
\Z
%%%%%%%%%%%%%%%%%%
\;,
\qquad
%%%%%%%%%%%%%%%%%%
\Tr\,(\dm)
=1
%%%%%%%%%%%%%%%%%%
\;.
\end{equation}
%_____________________________
%_____________________________
The normalization function
%_____________________________
%
% PARTITION FUNCTION
%_____________________________
\begin{equation}
\label{partition:function}
%%%%%%%%%%%%%%%%%%
\Z
=
\Tr\,
\e^{-\beta\Htot}
%%%%%%%%%%%%%%%%%%
\;,
\end{equation}
%_____________________________
%_____________________________
is called the {\em partition function}, and plays a central role in
several parts of the formalism.





many $\llangle \VQ \rrangle$ obtainable from the partition function by
differentiation.




For example: quantity $\VQ$ derivable from the Hamiltonian
%_____________________________
%
% X FROM H
%_____________________________
\begin{equation}
\label{XfromH}
%%%%%%%%%%%%%%%%%%
\VQ
=
\partial_{\bp}
\Ham_{\rm T}
%%%%%%%%%%%%%%%%%%
\;.
\end{equation}
%_____________________________
%_____________________________
EGs, $x$ from $-x\,F$, $\J$ from $-\J\cdot\B$





$\bp$ is some field-force parameter




average of $\VQ$
%
$\llangle \VQ \rrangle
=
\kT
\partial_{\bp}
\Z/\Z$
%
%_____________________________
%
% X AVERAGE
%_____________________________
\begin{equation}
\label{X:average}
%%%%%%%%%%%%%%%%%%
\llangle \VQ \rrangle
=
\Z'/\Z
%%%%%%%%%%%%%%%%%%
\;.
\end{equation}
%_____________________________
%_____________________________
$\kT\partial_{\bp}\Z=\partial_{(\beta\bp)}\Z\equiv\Z'$




susceptibility 
%_____________________________
%
% SUSCEPTIBILITY: DEF
%_____________________________
\begin{equation}
\label{chi:def}
%%%%%%%%%%%%%%%%%%
\X
=
\partial_{\bp}
\llangle \VQ \rrangle
=
\beta
\llangle \VQ \rrangle'
%%%%%%%%%%%%%%%%%%
\;.
\end{equation}
%_____________________________
%_____________________________



susceptibility from $\xi$-derivatives of $\Z$


$\X
=
\beta
\llangle \VQ \rrangle'$

%_____________________________
%
% SUSCEPTIBILITY: Z DERIVATIVES
%_____________________________
\begin{equation}
\label{X:Z:der}
%%%%%%%%%%%%%%%%%%
\X
=
\beta
\llangle \VQ \rrangle'
=
\beta
\bigg[
\frac{\Z''}{\Z}
-
\Big(
\frac{\Z'}{\Z}
\Big)^{2}
\bigg]
%%%%%%%%%%%%%%%%%%
\;,
\end{equation}
%_____________________________
%_____________________________



$\xi$-expansion of $\Z$
%_____________________________
%
% Z EXPANSION
%_____________________________
\begin{equation}
\label{Z:expansion}
%%%%%%%%%%%%%%%%%%
\Z
=
\Z_{0}
+
\xi
\Z_{1}
+
\half
\xi^{2}
\Z_{2}
+
\cdots
%%%%%%%%%%%%%%%%%%
\;.
\end{equation}
%_____________________________
%_____________________________



susceptibility in terms of $\xi$-expansion coefficients of $\Z$
%_____________________________
%
% SUSCEPTIBILITY: Z COEFFICIENTS
%_____________________________
\begin{equation}
\label{chi:Zi}
%%%%%%%%%%%%%%%%%%
\X
=
\beta
\bigg[
\frac{\Z_{2}}{\Z}
-
\Big(
\frac{\Z_{1}}{\Z}
\Big)^{2}
\bigg]
%%%%%%%%%%%%%%%%%%
\;.
\end{equation}
%_____________________________
%_____________________________



\subsection{perturbative treatment from Kubo's integral (interaction picture)}

total Hamiltonian
%_____________________________
%
% HAMILTONIAN
%_____________________________
\begin{equation}
\label{hamiltonian}
%%%%%%%%%%%%%%%%%%
\Htot
=
\Hs
+
\V
%%%%%%%%%%%%%%%%%%
\;,
\end{equation}
%_____________________________
%_____________________________


\subsection{susceptibility}

\subsubsection{general $\X$}

\subsubsection{$\X$ for ladder perturbations}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   PARAMAGNETS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   PARAMAGNETS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   PARAMAGNETS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   PARAMAGNETS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   PARAMAGNETS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   PARAMAGNETS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   PARAMAGNETS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{paramagnets}

\subsection{recovering standard expressions for paramagnets}

molecular magentism books

\subsubsection{Brillouin}

\subsubsection{anisotropic $S=1$ and $S=3/2$}

%_____________________________
%_____________________________
% chi-lo-tr-ran-S1.sh
%_____________________________
\begin{figure}[!tbh]
%
\centerline{
\includegraphics[width=10.cm]{chi-lo-tr-S1.eps}
}
\centerline{
\includegraphics[width=10.cm]{chi-ran-S1.eps}
}
\caption{%\small
%
Top panel:
%
Longitudinal and transverse susceptibility vs.\ temperature of $S=1$
spins with easy-axis anisotropy $\K=1$.
%
The Curie law $\SSp/3\kT$ (thin solid line) is approached by both $\Xlo$
 and $\Xtr$ at high $T$.
%
At low temperature $\Xlo$ goes over the 2-state (Ising) behavior
$S^{2}/\kT$ (dashed thin line), so in between the $\X$ increase is
faster than $1/\kT$.
%
The transverse susceptibility approaches $\Xtr=1/[2\K(1-1/2S)]$ at low $T$.
%
Bottom panel:
%
Susceptibilities plotted as $\kT \X$, including the average for axes
distributed at random, $\Xran=\frac{1}{3}\Xlo+\frac{2}{3}\Xtr$, which shows
deviation from isotropy at low temperatures.
%
}
\label{fig:X:S1:lo-tr-ran}
\end{figure}
%_____________________________
%_____________________________
%_____________________________


%_____________________________
%_____________________________
% chi-lo-tr-ran-S1p5.sh
%_____________________________
\begin{figure}[!tbh]
%
\centerline{
\includegraphics[width=10.cm]{chi-lo-tr-S1p5.eps}
}
\centerline{
\includegraphics[width=10.cm]{chi-ran-S1p5.eps}
}
\caption{%\small
%
Susceptibilities vs.\ temperature, as in
Fig.~\ref{fig:X:S1:lo-tr-ran}, but for $S=3/2$.
%
Top panel:
%
$\Xlo$ and $\Xtr$ vs.\ $T$, approaching the Curie law $\SSp/3\kT$ (thin
solid line) at high temperatures.
%
At low $T$, $\Xlo$ goes over the 2-state behavior $S^{2}/\kT$ (dashed
thin line), while $\Xtr$ approaches $\Xtr=1/[2\K(1-1/2S)]$.
%
Bottom panel:
%
The susceptibilities are plotted as $\kT \X$: longitudinal,
transverse, and the random axes average
$\Xran=\frac{1}{3}\Xlo+\frac{2}{3}\Xtr$.
%
}
\label{fig:X:S1p5:lo-tr-ran}
\end{figure}
%_____________________________
%_____________________________
%_____________________________

%_____________________________
%
% SUSCEPTIBILITY: UNIAXIAL: S=3/2
%_____________________________
\begin{eqnarray}
%%%%%%%%%%%%%%%%%%
\label{X:lo:unb:S1p5}
%%%%%%%%%%%%%%%%%%
\Xlo
&=&
%% \frac{\beta}{4}
%% \,
%% \frac
%% {1+10\,\e^{2\ds}+9\,\e^{4\ds}}
%% {(1+\e^{2\ds})^{2}}
%% =
\frac{\beta}{4}
\,
\frac
{\e^{-2\ds}+10+9\,\e^{+2\ds}}
{4\ch^{2}\ds}
%%%%%%%%%%%%%%%%%%
\\
\label{X:tr:unb:S1p5}
%%%%%%%%%%%%%%%%%%
\Xtr
&=&
\frac{\beta}{2(1+\e^{2\ds})}
\big[
3\,
K(2\ds)
+
2
\big]
%% =
%% \frac{3}{4\K}
%% \,
%% \big[
%% \thrm\ds
%% +
%% \tfrac{2}{3}\,
%% \ds\,
%% (1-\thrm\ds)
%% \big]
%%%%%%%%%%%%%%%%%%
\;.
\end{eqnarray}
%_____________________________
%_____________________________


\subsection{susceptibilities in superimposed external fields
  (longitudinal)}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%   SUPERPARAMAGNETS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%   SUPERPARAMAGNETS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%   SUPERPARAMAGNETS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%   SUPERPARAMAGNETS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%   SUPERPARAMAGNETS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%   SUPERPARAMAGNETS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%   SUPERPARAMAGNETS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{superparamagnets}

\subsection{longitudinal and transverse $\X$ for various $S$}

\subsection{the classical limit and the recovering of isotropy}

\subsection{from quantum to classical in $\X$ vs.\ $B$}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DISCUSSION   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DISCUSSION   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DISCUSSION   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DISCUSSION   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DISCUSSION   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DISCUSSION   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   DISCUSSION   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{discussion and conclusions}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   APENDICES   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newpage
\bigskip\bigskip
\centerline{\bf{\Large APPENDICES}}
\addcontentsline{toc}{section}{APPENDICES}
%OJO revtex

\appendix



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   ToDo & STUFF - ToDo & STUFF  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   ToDo & STUFF - ToDo & STUFF  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   ToDo & STUFF - ToDo & STUFF  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   ToDo & STUFF - ToDo & STUFF  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   ToDo & STUFF - ToDo & STUFF  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   ToDo & STUFF - ToDo & STUFF  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   ToDo & STUFF - ToDo & STUFF  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newpage
\section{ToDo \& stuff}


\begin{itemize}
%
\item 
appropiate connections to the big-spin community (if $\exists$)
%
\item 
%
easy way: focus on superparamagnets
%
\item 
$\Hs(\Sz)+\Vp(\Spm)$
%
\item 
$\Xlo$ , $\Xtr$ \& $\Xran=\tfrac{1}{3}\Xlo+\tfrac{2}{3}\Xtr$
%
\item 
alternative titles: 
\begin{enumerate}
%
\item 
{\bf equilibrium susceptibility of quantum (super)paramagnets: 
longitudinal \& transverse
}
\\
here we include the paramagnetic community (ions, EPR, etc)
%
\item 
{\bf thermal equilibrium response of big spin systems} 
\\ 
apparently more general, but would require more work including the
appropriate connections
%  
\end{enumerate}
%
\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   BIBLIOGRAPHY   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   BIBLIOGRAPHY   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   BIBLIOGRAPHY   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   BIBLIOGRAPHY   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%   BIBLIOGRAPHY   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%OJO revtex
\addcontentsline{toc}{section}{BIBLIOGRAPHY}

% You just need to give the path to your bibtex file
% (in case is not in the same folder)

% database.bib is the file with the database

%\bibliography{/path-to-your-folder/database.bib}
% EG
\bibliography{/home/jose/escritos/TEX/jlgarcia}

% in case is in the working directory
%\bibliography{database.bib} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   END  DOCUMENT   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   END  DOCUMENT   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   END  DOCUMENT   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   END  DOCUMENT   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%   END  DOCUMENT   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{document}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(70+spc)

.~%
%
\footnote{
%
%
} %END OF FOOTNOTE



